MIT at SemEval-2017 Task 10: Relation Extraction with Convolutional Neural Networks

Over 50 million scholarly articles have been published: they constitute a unique repository of knowledge. In particular, one may infer from them relations between scientific concepts, such as synonyms and hyponyms. Artificial neural networks have been recently explored for relation extraction. In this work, we continue this line of work and present a system based on a convolutional neural network to extract relations. Our model ranked first in the SemEval-2017 task 10 (ScienceIE) for relation extraction in scientific articles (subtask C).

==> tables/labeling_strategies.tex <==
 \begin{table*}[t]

\footnotesize
\centering
\setlength\tabcolsep{6.0pt}
\setlength{\extrarowheight}{3pt}
\setlength{\arraycolsep}{5pt}
\begin{tabular}{|c|ccc|ccc|}
\hline 
annotation & \multicolumn{6}{c|}{A is a hyponym of B (relation:hyponym\_of, arg1:A, arg2:B)} \tabularnewline
\hline 
order in text & \multicolumn{3}{c|}{... A ... B ...} & \multicolumn{3}{c|}{... B ... A ...}  \tabularnewline
\hline 
labeling strategy & relation & arg1 & arg2 & relation & arg1 & arg2 \tabularnewline
\hline 
correct order & hyponym\_of & A & B & hyponym\_of & A & B \tabularnewline
\hline 
\multirow{2}{*}{negative sampling} & hyponym\_of & A & B & hyponym\_of & A & B \tabularnewline
\cline{2-7} 
 & none & B & A & none & B & A \tabularnewline
\hline 
fixed order & hyponym\_of & A & B & hypernym\_of & A & B \tabularnewline
\hline 
\multirow{2}{*}{any order} & hyponym\_of & A & B & hypernym\_of & A & B \tabularnewline
\cline{2-7} 
 & hypernym\_of & B & A & hyponym\_of & B & A \tabularnewline
\hline 
annotation & \multicolumn{6}{c|}{A is a synonym of B (relation:synonym\_of, arg1:A, arg2:B)}  \tabularnewline
\hline 
order in text & \multicolumn{3}{c|}{... A ... B ...} & \multicolumn{3}{c|}{... B ... A ...}   \tabularnewline
\hline 
labeling strategy & relation & arg1 & arg2 & relation & arg1 & arg2 \tabularnewline
\hline 
correct/fixed & synonym\_of & A & B & synonym\_of & B & A \tabularnewline
\hline  
\multirow{2}{*}{neg.sampl./any} & synonym\_of & A & B & synonym\_of & B & A \tabularnewline
\cline{2-7} 
 & synonym\_of & B & A & synonym\_of & A & B \tabularnewline
\hline 
\end{tabular}
\caption{Various labeling strategies} 
\label{tab:labeling_strategies}
\end{table*}




==> tables/labeling_strategies2.tex <==

 \begin{table}[ht]
\footnotesize
\centering
\setlength\tabcolsep{3.0pt}
\setlength{\extrarowheight}{3pt}
\setlength{\arraycolsep}{3pt}
\begin{tabular}{|c|ccc|ccc|}
\hline 
annotation & \multicolumn{6}{c|}{A (arg1) is a hyponym (rel) of B (arg2)} \tabularnewline
\hline 
text order & \multicolumn{3}{c|}{... A ... B ...} & \multicolumn{3}{c|}{... B ... A ...}  \tabularnewline
\hline 
strategy & rel & arg1 & arg2 & rel & arg1 & arg2 \tabularnewline
\hline 
correct order & hyp & A & B & hyp & A & B \tabularnewline
\hline 
\multirow{2}{*}{neg. smp.} & hyp & A & B & hyp & A & B \tabularnewline
\cline{2-7} 
 & none & B & A & none & B & A \tabularnewline
\hline 
fixed order & hyp & A & B & hypr & A & B \tabularnewline
\hline 
\multirow{2}{*}{any order} & hyp & A & B & hypr & A & B \tabularnewline
\cline{2-7} 
 & hypr & B & A & hyp & B & A \tabularnewline
\hline \multicolumn{7}{c}{}  \tabularnewline
\hline
annotation & \multicolumn{6}{c|}{A (arg1) is a synonym (rel) of B (arg2)}  \tabularnewline
\hline 
text order & \multicolumn{3}{c|}{... A ... B ...} & \multicolumn{3}{c|}{... B ... A ...}   \tabularnewline
\hline 
strategy & rel & arg1 & arg2 & rel & arg1 & arg2 \tabularnewline
\hline 
correct order & syn & A & B & syn & A & B \tabularnewline
\hline  
\multirow{2}{*}{neg. smp.} & syn & A & B & syn & A & B \tabularnewline
\cline{2-7} 
 & syn & B & A & syn & B & A \tabularnewline
\hline
fixed order & syn & A & B & syn & B & A \tabularnewline
\hline  
\multirow{2}{*}{any order} & syn & A & B & syn & B & A \tabularnewline
\cline{2-7} 
 & syn & B & A & syn & A & B \tabularnewline
\hline 
\end{tabular}
\caption{Various labeling strategies} 
\label{tab:labeling_strategies}
\end{table}



